Vulnerability Scanners for Ethereum Smart Contracts: A Large-Scale Study

Ethereum smart contracts, which are autonomous decentralized applications on the blockchain that manage assets often exceeding millions of dollars, have become primary targets for cyberattacks. In 2023 alone, such vulnerabilities led to substantial financial losses exceeding a billion of US dollars. To counter these threats, various tools have been developed by academic and commercial entities to detect and mitigate vulnerabilities in smart contracts. Our study investigates the gap between the effectiveness of existing security scanners and the vulnerabilities that still persist in practice. We compiled four distinct datasets for this analysis. The first dataset comprises 77,219 source codes extracted directly from the blockchain, while the second includes over 4 million bytecodes obtained from Ethereum Mainnet and testnets. The other two datasets consist of nearly 14,000 manually annotated smart contracts and 373 smart contracts verified through audits, providing a foundation for a rigorous ground truth analysis on bytecode and source code. Using the unlabeled datasets, we conducted a comprehensive quantitative evaluation of 17 vulnerability scanners, revealing considerable discrepancies in their findings. Our analysis of the ground truth datasets indicated poor performance across all the tools we tested. This study unveils the reasons for poor performance and underscores that the current state of the art for smart contract security falls short in effectively addressing open problems, highlighting that the challenge of effectively detecting vulnerabilities remains a significant and unresolved issue.

==> text/table.tex <==
\begin{table*}%[ht!]
	\centering
	\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%NO \Circle\ 
%YES \CIRCLE 
%MORE \dowcirc
\hline
\multirow{2}{*}{\thead{Metrics}} & \multicolumn{5}{l|}{ \thead{Static Analysis}} & \multicolumn{7}{l|}{\thead{Symbolic Execution}} & \multicolumn{4}{l|}{\thead{Fuzzing}} & \multicolumn{2}{l}{\thead{Machine Learning}} \\ \cline{2-19} 
                    & Slither     & EtherTrust     & Vandal     & MadMax     & SmartCheck   &  Maian   & Oyente   & Artemis  &  Osiris   & Securify2  & Mythril  & TeEther  &  ILF & ConFuzzius & Smartian & sFuzz & GNNSCVulDetector & ESCORT \\ \hline
Suicidal           &   \Circle\   &   \Circle\     & \CIRCLE    &  \Circle\  &  \Circle\    & \CIRCLE  & \Circle\ & \Circle\ & \Circle\  & \CIRCLE    & \CIRCLE  & \Circle\ & \Circle\ & \CIRCLE  & \CIRCLE  & \Circle\ & \Circle\ & \CIRCLE\ \\ %\hline
%Empty              &   \Circle\   &   \Circle\     & \Circle\   &  \Circle\  &  \Circle\    & \Circle\ & \Circle\ & \Circle\ & \Circle\  & \Circle\   & \Circle\ & \Circle\ & \Circle\ & \Circle\ & \Circle\ & \Circle\ & \Circle\ & \Circle\ \\ \hline
Reentrancy         &   \dowcirc   &   \Circle\     & \CIRCLE    &  \Circle\  &  \Circle\    & \Circle\ & \CIRCLE  & \CIRCLE  & \CIRCLE   & \dowcirc   & \CIRCLE  & \Circle\ & \Circle\ & \CIRCLE  & \CIRCLE  & \Circle\ & \Circle\ & \CIRCLE  \\ %\hline
Reentrancy Bad     &   \CIRCLE   &   \Circle\     & \Circle    &  \Circle\  &  \Circle\    & \Circle\ & \Circle  & \Circle  & \Circle    & \CIRCLE    & \Circle  & \Circle\ & \Circle\ & \Circle  & \Circle  & \Circle\ & \Circle\ & \Circle  \\ %\hline
Reentrancy No Eth  &   \CIRCLE   &   \Circle\     & \Circle    &  \Circle\  &  \Circle\    & \Circle\ & \Circle  & \Circle  & \Circle    & \CIRCLE    & \Circle  & \Circle\ & \Circle\ & \Circle  & \Circle  & \Circle\ & \Circle\ & \Circle  \\ %\hline
Reentrancy Benign  &   \CIRCLE   &   \Circle\     & \Circle    &  \Circle\  &  \Circle\    & \Circle\ & \Circle  & \Circle  & \Circle    & \CIRCLE    & \Circle  & \Circle\ & \Circle\ & \Circle  & \Circle  & \Circle\ & \Circle\ & \Circle  \\ %\hline
ToD                &   \Circle\   &   \Circle\     & \Circle\   &  \Circle\  &  \Circle\    & \Circle\ & \Circle\ & \CIRCLE & \CIRCLE   & \dowcirc   & \Circle\ & \Circle\ & \Circle\ & \CIRCLE\ & \Circle\ & \Circle\ & \Circle\ & \Circle\ \\ %\hline
Arithmetic Bug     &   \Circle\   &   \Circle\     & \Circle\   &  \Circle\  &  \Circle\    & \Circle\ & \Circle\ & \dowcirc\ & \dowcirc\  & \Circle\   & \Circle\ & \Circle\ & \Circle\ & \dowcirc\ & \CIRCLE\ & \Circle\ & \Circle\ & \Circle\ \\ \hline
\end{tabular}
\end{adjustbox}
%\vspace{1.5em}
   \caption{Overview of vulnerability scanners with detectable vulnerability types on source code.\christoph{all except escort allow the usage of source code (they just compile the code like Vandal)}\todo{make it look nicer (\url{https://people.inf.ethz.ch/markusp/teaching/guides/guide-tables.pdf})}}   \label{tab:overview_tools_source}
   %\vspace{-2.5em}
\end{table*}
